Learning Monocular Reactive UAV Control in Cluttered Natural Environments

Autonomous navigation for large Unmanned Aerial Vehicles (UAVs) is fairly straight-forward, as expensive sensors and monitoring devices can be employed. In contrast, obstacle avoidance remains a challenging task for Micro Aerial Vehicles (MAVs) which operate at low altitude in cluttered environments. Unlike large vehicles, MAVs can only carry very light sensors, such as cameras, making autonomous navigation through obstacles much more challenging. In this paper, we describe a system that navigates a small quadrotor helicopter autonomously at low altitude through natural forest environments. Using only a single cheap camera to perceive the environment, we are able to maintain a constant velocity of up to 1.5m/s. Given a small set of human pilot demonstrations, we use recent state-of-the-art imitation learning techniques to train a controller that can avoid trees by adapting the MAVs heading. We demonstrate the performance of our system in a more controlled environment indoors, and in real natural forest environments outdoors.

==> experiments.tex <==
\section{Experiments}
\label{sec.experiments}

\subsection{Setup}

We use the Parrot ARDrone as our robotic platform \cite{parrotardrone}. This
is a cheap, commercially available quadrotor, weighing
~420g and size ~0.3mx0.3m. It
has a front-facing camera of 320x240 pixels and 93-degree field of view, an
ultrasound altimeter, a lower resolution down-facing camera and onboard
IMU. The drone's onboard controller stabilizes the drone and allows
control of the UAV through high-level desired velocity commands
(forward-backward, left-right, up-down velocities, and rotational yaw
velocity) and can reach a maximum velocity of around $5$m/s. These commands are
sent through wifi and the drone also streams the 320x240 images from the
camera through wifi at around $10$-$15$ Hz. This allows us to control the
drone on
a separate computer that receives and processes the images from the drone, and
then sends back commands to the drone at around $10$Hz. We use
the Robotic Operating System (ROS) \cite{ros} and the ROS ARDrone Driver
\cite{ardronedriver} to interface/communicate with the drone from the
computer.

% \begin{figure}[!htbp]
%   \centering
%   \mbox{
%     \subfloat[Motion-capture arena indoor setup]{\label{indoor_setup}\includegraphics[width=1.0\linewidth]{figures/drone_indoor_setup.png}}
%   }
%   \mbox{
%     \subfloat[Outdoor groundstation setup]{\label{outdoor_setup}\includegraphics[width=1.0\linewidth]{figures/outdoor_setup.png}}
%   } 
%   \mbox{
%   \subfloat[Long range wifi antenna]{\label{robot_on_map}\includegraphics[width=1.0\linewidth]{figures/wifi_outdoors.png}}
%   }
% \caption{Indoor and outdoor setup}
% \label{setup_figure}
% \end{figure}


\subsection{Indoor Experiments}

We first tested our approach indoors in a motion capture arena. We use fake indoor trees as obstacles and camouflage to hide background clutter (see Figure \ref{dagger_indoor_setup}). While this is a very controlled environment that lacks many of the complexities of real outdoor scenes, this allowed us to obtain better quantitive results to determine the effectiveness of our approach.

The motion capture system is only used to track the drone and adjust its heading so that it is always heading straight towards a given goal location. The drone moves at a fixed velocity of 0.25m/s and we seek to learn a controller that swerves left or right to avoid trees on the way to the goal only based on the observed camera images.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/dagger_indoor_setup.png}
	\caption{Indoor setup in motion capture arena with fake plastic trees and camouflage in background.}
	\label{dagger_indoor_setup}
\end{figure}

We used DAgger to train the controller over 3 iterations of training, and at each iteration, we used $11$ fixed scenarios to collect training data. There was $1$ scenario with no obstacles, $3$ with $1$ obstacle and $7$ with $2$ obstacles (see Figure \ref{dagger_indoor_scenario}). We learned a linear controller using ridge regression that attempts to predict the left-right velocity as a linear function of the observed visual features extracted from the camera image.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/39IndoorScenario.png}
	\caption{The $11$ obstacle arrangements used to train Dagger for every iteration in the motion capture arena. The drone and star indicate the start and goal location respectively.}
	\label{dagger_indoor_scenario}
\end{figure}

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.7\textwidth]{figures/37MocapToGoal.png}
%	\caption{The drone controller learns to move straight towards the goal location while swerving to avoid trees in the way.}
%	\label{dagger_mocap_to_goal}
%\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/dagger_traj_comparison.png}
	\caption{The rightmost trajectory is the initial demonstrated trajectory by the human expert flying the UAV looking at the front-facing camera stream. The short trajectories in red show the results of the controllers learnt in the first and second iterations which collide. The third iteration controller no longer collides and is similar to the demonstrated trajectory.}
	\label{dagger_traj_comparison}
\end{figure}

Figure \ref{dagger_traj_comparison} shows the trajectories taken by the UAV in the mocap arena after each iteration of training on one of the particular scenario. In the first iteration, the green trajectory to the farthest right is the demonstrated trajectory by the human expert pilot. The short red and orange trajectories are the trajectories taken by the UAV after the $1^{st}$ and $2^{nd}$ iterations were completed. Note that both collide with the obstacle. After the $3^{rd}$ iteration, however, it learned a trajectory which avoids both obstacles. Figure \ref{dagger_interventions} shows the percentage of scenarios where the pilot had to intervene for the learned controller after each iteration. The interventions required decrease between iterations and after 3 iterations, there was no need to intervene as the UAV successfully avoided all the obstacles on all scenarios.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/dagger_interventions.png}
	\caption{Percentage of scenarios the pilot had to intervene and the imitation loss (average squared error in controls of controller to human expert on hold-out data) after each iteration of Dagger. After 3 iterations, there was no need for the pilot to intervene and the UAV could successfully avoid all obstacles.}
	\label{dagger_interventions}
\end{figure}



\subsection{Indoor Experiments}

We first tested our approach indoors in a motion capture arena. We use fake indoor trees as obstacles and camouflage to hide background clutter (see Figure \ref{dagger_indoor_setup}). While this is a very controlled environment that lacks many of the complexities of real outdoor scenes, this allowed us to obtain better quantitive results to determine the effectiveness of our approach.

The motion capture system is only used to track the drone and adjust its heading so that it is always heading straight towards a given goal location. The drone moves at a fixed velocity of 0.25m/s and we seek to learn a controller that swerves left or right to avoid trees on the way to the goal only based on the observed camera images.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/dagger_indoor_setup.png}
	\caption{Indoor setup in motion capture arena with fake plastic trees and camouflage in background.}
	\label{dagger_indoor_setup}
\end{figure}

We used DAgger to train the controller over 3 iterations of training, and at each iteration, we used $11$ fixed scenarios to collect training data. There was $1$ scenario with no obstacles, $3$ with $1$ obstacle and $7$ with $2$ obstacles (see Figure \ref{dagger_indoor_scenario}). We learned a linear controller using ridge regression that attempts to predict the left-right velocity as a linear function of the observed visual features extracted from the camera image.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/39IndoorScenario.png}
	\caption{The $11$ obstacle arrangements used to train Dagger for every iteration in the motion capture arena. The drone and star indicate the start and goal location respectively.}
	\label{dagger_indoor_scenario}
\end{figure}

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.7\textwidth]{figures/37MocapToGoal.png}
%	\caption{The drone controller learns to move straight towards the goal location while swerving to avoid trees in the way.}
%	\label{dagger_mocap_to_goal}
%\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/dagger_traj_comparison.png}
	\caption{The rightmost trajectory is the initial demonstrated trajectory by the human expert flying the UAV looking at the front-facing camera stream. The short trajectories in red show the results of the controllers learnt in the first and second iterations which collide. The third iteration controller no longer collides and is similar to the demonstrated trajectory.}
	\label{dagger_traj_comparison}
\end{figure}

Figure \ref{dagger_traj_comparison} shows the trajectories taken by the UAV in the mocap arena after each iteration of training on one of the particular scenario. In the first iteration, the green trajectory to the farthest right is the demonstrated trajectory by the human expert pilot. The short red and orange trajectories are the trajectories taken by the UAV after the $1^{st}$ and $2^{nd}$ iterations were completed. Note that both collide with the obstacle. After the $3^{rd}$ iteration, however, it learned a trajectory which avoids both obstacles. Figure \ref{dagger_interventions} shows the percentage of scenarios where the pilot had to intervene for the learned controller after each iteration. The interventions required decrease between iterations and after 3 iterations, there was no need to intervene as the UAV successfully avoided all the obstacles on all scenarios.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/dagger_interventions.png}
	\caption{Percentage of scenarios the pilot had to intervene and the imitation loss (average squared error in controls of controller to human expert on hold-out data) after each iteration of Dagger. After 3 iterations, there was no need for the pilot to intervene and the UAV could successfully avoid all obstacles.}
	\label{dagger_interventions}
\end{figure}

\subsection{Feature Evaluation}

In the current implementation we transmit images from the drone to the
workstation at 15-30~Hz, and compute the entire set of features at 15~Hz. For our current flight speed of approx. 1~m/s and
command rate of 10~Hz, this is fast enough. We verified the robustness of the
features by training and testing under very different conditions as
illustrated in Figure~\ref{fig:generalize}.

\begin{figure}[htbp]
	\centering
\begin{tabular}{cc}
	\includegraphics[width=0.7\linewidth]{figures/14train.png} \\
	\includegraphics[width=0.7\linewidth]{figures/14test.png} 
\end{tabular}
	\caption{Example of different observations used at training time (top) and test time (bottom) to validate the robustness and generalization power of the visual features.}
	\label{fig:generalize}
\end{figure}

An ablative analysis on the data shows that the structure tensor features are most important for proper collision avoidance, followed by optical flow features. While structure tensor features mainly fire due to texture in the background (indicating free space), strong optical flow vectors correspond to close objects. Figure \ref{fig:feat-arrows} shows the contribution of each of the features at different window centers in the image, for a particular example where the predictor commanded a hard left turn (numerical value: 0.47, positive values indicate a left command). The breakdown among the different features is the following. Radon: 0.01, structure tensor: 0.38, laws: 0.05, flow: 0.05, history: -0.02.

%\begin{figure*}[htbp]
%	\centering
%\begin{tabular}{cc}
%	\includegraphics[width=0.2\textwidth]{frame17-radon} 
%	\includegraphics[width=0.2\textwidth]{frame17-harris} 
%	\includegraphics[width=0.2\textwidth]{frame17-laws} 
%	\includegraphics[width=0.2\textwidth]{frame17-flow} 
%	\includegraphics[width=0.2\textwidth]{frame17-all}
%\end{tabular}

\begin{figure*}
	\centering
	\subfloat[Radon]{ \includegraphics[width=0.19\textwidth]{frame17-radon} }~ 
	\subfloat[Structure Tensor]{ \includegraphics[width=0.19\textwidth]{frame17-harris} }~
	\subfloat[Laws]{ \includegraphics[width=0.19\textwidth]{frame17-laws} }~ 
	\subfloat[Flow]{ \includegraphics[width=0.19\textwidth]{frame17-flow} }~
	\subfloat[All Features]{ \includegraphics[width=0.19\textwidth]{frame17-all} }

	\caption{Visualization of the contribution of the different features to the predicted control. The overall control was a hard left command. The arrows show the contribution of a given feature at every window. Structure tensor features have the largest contribution in this example, while Radon has the least.}
	\label{fig:feat-arrows}
\end{figure*}

\subsection{Outdoor Experiments}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{dagger_improvement}
%\caption{The above plots show that as Dagger progresses the number of
%  interventions per unit distance and imitation loss with respect to the human
%  expert goes down.}
%\label{fig.dagger_improvement}
%\end{figure}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{overhead_map}
%\caption{Shows the actual trajectories taken by Dagger at each iteration for
%  different starting locations. The trajectories are formatted by iteration
%  number. As iterations increase they can avoid obstacles for a longer distance. }
%\label{fig.overhead_map}
%\end{figure}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{system_diagram}
%\caption{Shows our overall system architecture and the various latencies.}
%\label{fig.system_diagram}
%\end{figure}

After testing thoroughly indoors in the motion capture arena to validate the approach, we conducted experiments outdoors to test more real-world scenarios. As we couldn't use to motion capture system outdoors to make the drone head toward a specific goal location, we simply made the drone always move forward at a fixed speed and aimed to learn a controller that would swerve left or right to avoid any trees on the way while maintaining initial heading. Again, we attempted to learn a linear controller using ridge regression that would predict the left-right velocity as a linear function of observed visual features. Training and testing was conducted in forest areas while restraining the aircraft using a very light-weight tether. 

For the outdoor experiments the drone was operated autonomously over ***km for a net autonomous flight time duration of *** minutes. Our training dataset comprised two categories of test regions - a sparser park and a dense wooded region with a tree density of 0.8 trees per 10 square meters. The expectation for test performance as per ***cite reference?*** was that an increase in tree density would impact our maximum forward velocity negatively. In the following discussion we shall evaluate performance of DAgger in these two training regions.

For the purpose of classification of data regarding avoiding trees, the human labellers adhered to the following criteria 
\begin{itemize}
\item A tree is \textit{avoided} when the drone can see the tree pass from within its field of view to the edge of the image
\item A \textit{useful input} is a velocity command (or a series of smaller continuous commands) output by DAgger above a threshold depending on current forward velocity which causes the drone to significantly move to avoid a tree. No condition is imposed on the input being successful in avoiding a tree.
\item A \textit{non useful input} is correspondingly any command velocity greater than the above mentioned threshold that does not assist in avoiding a tree. Examples would be the drone turning while in open terrain and heading into a tree after an initial command of heading away
\item Trees are passed through the middle if the separation between the two trees is within a three meters and the drone can see both trees in its field of view moving towards the corresponding edges. These trees are not counted in the trees avoided by moving left or right.

%***Mention two sets of tests, a sparser training region and a denser region, %and develop the argument as a continuous progress from a slower speed and %lower resolution to a greater forward speed and higher camera resolution***

\end{itemize}

\subsubsection{Sparser test region}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/48testSite.png}
	\caption{The two test sites and the main training site for the sparser dataset}
	\label{dagger_sites}
\end{figure}


Figure  shows an overhead view of the main training area and the two test areas.
***include below total amount of training flight data in experiment, or per iteration, and specify exact number of iterations*** ***also should try to include tree density of train/test sites and overall collision frequency***

The controller was trained with DAgger for four iterations in the training area and was tested in the two marked test areas \ref{dagger_sites}. The resulting controller performed well in the test areas and was successfully able to avoid trees, even in densely forested areas. In particular, the drone was able to fly autonomously without crashing in any trees over a 100m distance in one of the test area, reaching the limit of our communication range for the tests. A video shows the behavior of the learned controller during one of those runs ***cite***.

***Fancy Analysis for May 5 comes here***

The learned controller is however not perfect and several failure modes were observed. After the first iteration of training, the drone sometimes collided with large trees even when they were in plain view (Figure~\ref{dagger_atypical_failures_first}). At later iterations however, this rarely occured (Figure~\ref{dagger_atypical_failures_third}). On the other hand, we observed that the drone had more difficulty detecting branches or bushes and observed a number of failures that would occur throughout the iterations of training. The fact that fewer of such obstacles were seen in the training data coupled with the inability of the expert piloting the drone to distinguish them from the background contributed to the difficulty of dealing with these obstacles. 
We proposed that better visual features or improved camera resolution might help, as small branches often can't be seen from the low resolution 320x240 pixel image. But, as expected, we found that the narrow field-of-view was the largest contributor to failures of the reactive approach (Figure~\ref{dagger_nfov_failures}). The typical case is when the learned controller avoids a tree, and as it turns a new tree comes into view. This may cause the controller to turn in a way such that it collides sideways into the last tree it just avoided. This problem inevitably afflicts purely reactive controllers. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/53-55atypicalFailures.png}
	\caption{Some scenarios where Dagger failed in the first iteration.}
	\label{dagger_atypical_failures_first}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/53-55atypicalFailures3rdIteration_horiz.png}
	\caption{Some scenarios where Dagger failed in the third iterations.}
	\label{dagger_atypical_failures_third}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/53-55NFOVFailures.png}
	\caption{The most common failures are due to the narrow field of view of the camera where some trees barely appear to one side of the camera or are just hidden outside the view. When the UAV turns to avoid a visible tree in a bit farther away it collides with the tree to the side}
	\label{dagger_nfov_failures}
\end{figure}

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.5\linewidth]{58NFVOVIssue.png}
%	\caption{Illustration of the narrow field of view problem in Dagger. The UAV swerves to avoid a tree in view but collides with the tree which it cannot see.}
%	\label{dagger_nfov_failures_principle}
%\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/57FOVs}
	\caption{Field of view comparison.}
	\label{FOVs}
\end{figure}


\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/plots/direction_passing_may}
	\caption{Comparision of trees passed over iterations.}
	\label{passed_may}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/plots/trees_avoided_may}
	\caption{Scatter plot of trees avoided (passively and actively) over time of flight. ***This should be distance for easy comparision with the next plot*** Here the slope of the plots for both Human and DAgger are different, since the drone was landed whenever the operator entered an open area, while DAgger was allowed to run in those regions.}
	\label{scatter_may}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/plots/flight_time_may}
	\caption{Diagram showing the average flight time between interventions}
	\label{time_may}
\end{figure}


\subsubsection{Dense test region}

The second testing region for outdoor experiments was conducted in a thickly wooded region in a local forest. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/plots/direction_passed_sep}
	\caption{Comparision of trees passed over iterations. Notice change in relative preference of DAgger from the second to third iteration. This reflects the conscious choice of the pilot to avoid trees on the right in the training iteration}
	\label{passed_sep}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/plots/trees_avoided_sep}
	\caption{Scatter plot of trees avoided (passively and actively) over time of flight. ***This should be distance for easy comparision with the previous plot*** Here the slope of the plots for both Human and DAgger are identical}
	\label{scatter_sep}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/plots/flight_time_sep}
	\caption{Diagram showing the average flight time between interventions}
	\label{time_sep}
\end{figure}

Active - Passive Ratio of passed trees:\\
Human : 66.4 \% Active, 33.6 \% Passive\\
DAgger - Overall : 61.9 \% Active, 38.1 \% Passive\\

Passing trees left -right - middle:\\
Human : 35.4 \% Left, 21.2 \% Right, 40.7 \% Middle \\
DAgger - Overall : 35.4 \% Left, 41.6 \% Right, 21.8\% Middle\\

Ratio of Useful Controls\\
Human: 94.73 \%\\
DAgger - Overall: 50.5 \%\\
DAgger - After Iter 1: 54.2 \%\\
DAgger - After Iter 2: 60.0 \%\\
DAgger - After Iter 3: 40.5 \%\\

Types of Crash Analysis\\
Human: Visible Large Tree: 0\%, Visible Thin Tree 16.7\%, Narrow FOV: 33.3\%, Folliage: 33.3\%, Branches 16.7 \%, Misc: 0\%\\
DAgger After Iter 1: Visible Large Tree: 33.3\%, Visible Thin Tree 8.3\%, Narrow FOV: 50\%, Folliage: 0\%, Branches 0\%, Misc: 8.3\%\\
DAgger After Iter 2: Visible Large Tree: 35.3\%, Visible Thin Tree 23.5\%, Narrow FOV: 23.5\%, Folliage: 5.9\%, Branches 11.8 \%, Misc: 0\%\\
DAgger After Iter 3: Visible Large Tree: 27.3\%, Visible Thin Tree 9.1\%, Narrow FOV: 36.4\%, Folliage: 9.1\%, Branches 18.2 \%, Misc: 0\%\\

Flight Time Per Crash:\\
Human: 59.81s\\
DAgger After Iter 1: 21.62s\\
DAgger After Iter 2: 21.59s\\
DAgger After Iter 3: 30.26s\\

Flight Time Per Non FOV Crash\\
Human: 89.71s\\
DAgger After Iter 1: 43.24s\\
DAgger After Iter 2: 29.44s\\
DAgger After Iter 3: 45.28s\\

Flight Time Per Non FOV \& Non Branch+Folliage Crash\\
Human: 358.86s\\
DAgger After Iter 1: 54.05s\\
DAgger After Iter 2: 40.48s\\
DAgger After Iter 3: 90.77s\\

\subsubsection{Discussion of Outdoor Results}

The issues presented in the previous two subsections may be addressed by two approaches: first, imitation learning methods that integrate a small amount of memory may enable the simplest failure cases to be overcome without resorting to a complete and expensive mapping of the environment; second, the biologically-inspired approach is to simply ensure a wider field of view for the camera system. Figure \ref{FOVs} shows the comparison of the field of view of a pigeon and an owl against the drone. A case can be made for having increased field of view.



==> system.tex <==
%\section{UAV \& Control Infrastructure}

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.8\linewidth]{figures/drone.png}
%	\caption{Our current UAV, the Parrot AR.Drone \cite{parrotardrone}.}
%	\label{figDrone}
%\end{figure}
%
%We use the Parrot AR.Drone as our robotic platform (see Figure~\ref{figDrone}) \cite{parrotardrone}. This is a cheap and commercially available quadrotor being sold at \$300, weighting ~420g and measuring ~0.3mx0.3m in dimensions. In terms of sensing, the drone has a front-facing camera of 320x240 pixels with a 93-degree field of view, an ultrasound altimeter, a lower resolution down-facing camera and onboard IMU. The drone's onboard controller already stabilizes the drone and allow control of the UAV through high-level desired velocity commands (forward-backward, left-right, up-down velocities, and rotational yaw velocity) and can reach a maximum velocity of around 5m/s. These commands are sent through wifi and the drone also streams the 320x240 images from the camera through wifi at around 10-15 Hz. This allows us to control the drone on a seperate computer that receives and process the images from the drone, and then sends back commands to the drone at around 10Hz. We use the Robotic Operating System (ROS) \cite{ros} and the ROS ARDrone Driver \cite{ardronedriver} to interface/communicate with the drone from the computer.
